Enabling High-Quality In-the-Wild Imaging from Severely Aberrated Metalens Bursts

We tackle the challenge of robust, in-the-wild imaging using ultra-thin nanophotonic metalens cameras. Meta-lenses, composed of planar arrays of nanoscale scatterers, promise dramatic reductions in size and weight compared to conventional refractive optics. However, severe chromatic aberration, pronounced light scattering, narrow spectral bandwidth, and low light efficiency continue to limit their practical adoption. In this work, we present an end-to-end solution for in-the-wild imaging that pairs a metalens several times thinner than conventional optics with a bespoke multi-image restoration framework optimized for practical metalens cameras. Our method centers on a lightweight convolutional network paired with a memory-efficient burst fusion algorithm that adaptively corrects noise, saturation clipping, and lens-induced distortions across rapid sequences of extremely degraded metalens captures. Extensive experiments on diverse, real-world handheld captures demonstrate that our approach consistently outperforms existing burst-mode and single-image restoration techniques.These results point toward a practical route for deploying metalens-based cameras in everyday imaging applications.

==> figures/abla_rebut_align.tex <==

 \begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/assets/fig_rebut1_1_align2.pdf}
    \caption{\textit{Restoration with mis-alignment.} Our restoration network performs well in the case of moderately misaligned bursts (LoFTR \cite{sun2021loftrdetectorfreelocalfeature}, second row) while leads to slight blurring in case of higher misalignment (HDR+ \cite{hasinoff2016burst}, third row). On the other hand, precise alignment using our proposed alignment module (first row) leads to sharper image features.  
    }
    \label{fig:rebut_align}
    % \vspace{-2mm}
\end{figure*}

==> figures/abla_rebut_lsat.tex <==

 \begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/assets/fig2_rebut_wacv_lsat.pdf}
    \caption{\textit{Significance of real-world adaptation.} Our model trained just on the synthetic dataset performs poorly in HDR scenes in the real world visualized by the incorrect burst fusion maps. We refine them through unsupervised finetuning using saturation maps computed directly from the real burst  frames leading to higher quality fusion maps. 
    }
    \label{fig:rebut_lsat}
    % \vspace{-2mm}
\end{figure*}

==> figures/multi_scale.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/assets/fig_rebut1_2_multi.pdf}
      \caption{\textit{Multi-scale displacement fusion.} The first row shows the reference frame, target frame, and their displacement map. The subsequent rows visualize flow fields across pyramid levels (k = 0, 1, 2), where arrow direction encodes motion direction and arrow length/color encode displacement magnitude.}
    \label{fig:rebut_multi}
    % \vspace{-2mm}
\end{figure}

==> figures/teaser.tex <==
% \twocolumn[{%
%   \renewcommand\twocolumn[1][]{#1}%
%   \maketitle
%   \vspace{-1.1cm}
%   \begin{center}
%    \centering
%     \small
%    \includegraphics[width=0.95\textwidth]{figures/assets/figure_teaser_hdr.pdf}
%    \vspace{-2mm}
%    \captionof{figure}{A prototype ultra-lightweight metalens camera (left) compared to conventional refractive lens systems produces degraded burst images (center) with blur, noise, and over-saturation due to design constraints and limited dynamic range. While state-of-the-art restoration methods like Restormer fail due to poor generalization, our adaptive burst fusion strategy effectively overcomes these limitations.
%    % Ultra-lightweight single-layered metalens cameras exhibiting images with severe blurriness and low dynamic range can be improved significantly when paired with a joint deblurring and HDR reconstruction neural network. Real-world hand-held bursts captured under unknown exposure levels are first aligned robustly using pyramid feature matching and then fused together in a single step. In-the-wild results show significant improvements over previous methods on the new MetaHDR benchmark.
%    }
%    \label{fig:teaser}
%   \end{center}%
%  }]

 \begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{images/figure_teaser.pdf}
    \caption{\textbf{(a)} Comparing (left) against a refractive convex lens our metalens is orders of magnitude thinner; We mount the camera module on a Jetson Nano Orin edge device for inference. \textbf{(b)} We demonstrate HDR reconstruction as an avenue for our burst restoration pipeline. \textbf{(c)} We show real-time video restoration on our handheld metalens camera with better quality than previous state-of-the-art methods.
    }
    % \todo{Replace the tripod image with someone holding the tripod to justify handheld capture. Also replace baselines with a metalens recovery method and a img recovery algo. Better if both look bad to make the teaser more interesting.}
    \label{fig:teaser}
\end{figure*}

==> tables/table_ablation_align.tex <==


\setlength{\tabcolsep}{10pt}
\begin{table}[t]
\centering
\scriptsize
\caption{\textit{Ablation study on model design.} For each experiment, the base starting model was obtained from the trained checkpoint of \cref{tab:comparison}. Base model number is \underline{underlined}.}
\label{tab:ablation}
% \resizebox{\columnwidth}{!}{%
\def\arraystretch{1.05}%
\begin{tabular}{lcc}
\toprule
% \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{Non-Reference Metrics}} \\
% \cmidrule{2-5}
Experiments   & PSNR $\uparrow$ & LPIPS $\downarrow$  \\
\midrule
Number of burst frames (5 \textbar 7 \textbar 10)  & \underline{26.5} \textbar 26.7 \textbar 26.9 & \underline{0.25} \textbar 0.24 \textbar 0.24 \\
Channel depth (16 \textbar  20 \textbar  24) & 24.3 \textbar \underline{26.5} \textbar 26.3 & 0.29 \textbar \underline{0.25} \textbar 0.25  \\
Transformers per AFB (1 \textbar  2 \textbar  3) & 25.8 \textbar \underline{26.5} \textbar 26.5 & 0.28 \textbar \underline{0.25} \textbar 0.26  \\
w/o. (APCU \textbar  AFB) & 24.7 \textbar 24.4 & 0.38 \textbar 0.40 \\
w/o. APCU \& w/o. AFB  & 24.2 & 0.41 \\
% HDR-USRNet \cite{} & -- & -- & -- \\
w/o. $I_{res}$  & 19.9 & 0.47 \\
% \midrule
% \rowcolor{green!20} \textbf{Ours} & \textbf{23.75} & \textbf{4.31} & \textbf{28.77} \\
\bottomrule
\end{tabular}%
\vspace{-6mm}
% }
\label{tab:ablat_align}
\end{table}

==> tables/table_alignment.tex <==
% \setlength{\tabcolsep}{2.5pt}  
% \begin{table}[h]
% \scriptsize
% \centering
% \caption{Comparison of different models under various exposure conditions (with standard deviations).}
% \begin{tabular}{lcccccc}
% \toprule
% Model & \begin{tabular}{c}
%      Median   \\
%      Error 
% \end{tabular}  $\downarrow$  & \begin{tabular}{c}
%      Cosine   \\
%      Similarity  
% \end{tabular}  $\uparrow$ & Std Dev $\downarrow$ &\begin{tabular}{c}
%      MSE   \\
%      Error 
% \end{tabular} $\downarrow$   & Std Dev $\downarrow$ \\
% \midrule
% \multicolumn{6}{c}{\emph{Low Exposure - 48 raw frames}} \\
% \midrule
% \cite{10.5555/1623264.1623280}
%    & 129.31 & 0.02 & 0.71 & 109.35 & 28.02 \\
% HDRPLUS \cite{10.1145/2980179.2980254}       & 53.65  & 0.10 & 0.70 & 44.92  & 13.10 \\
% Superres \cite{ipol.2023.460}      & 53.80  & 0.11 & 0.70 & 45.00  & 13.09 \\
% RAFT \cite{teed2020raftrecurrentallpairsfield}           & 27.14  & 0.54 & 0.68 & 63.70  & 61.19 \\
% PWC-Net \cite{}       & - & - & - & -  & - \\
% SPyNet \cite{}          & -  & - & - & -  & - \\
% LoFTR \cite{sun2021loftrdetectorfreelocalfeature}          & 3.75   & 0.94 & 0.19 & 3.94   & 3.04 \\
% \rowcolor{green!20} Our Model    & 1.71   & 0.99 & 0.06 & 1.40   & 1.15 \\
% \midrule
% \multicolumn{6}{c}{\emph{Medium Exposure - 48 raw frames}} \\
% \midrule
% \cite{10.5555/1623264.1623280}   & 22.26 & 0.41 & 0.64 & 15.86  & 5.40 \\
% HDRPLUS \cite{10.1145/2980179.2980254}       & 7.05  & 0.76 & 0.45 & 8.77   & 3.66 \\
% Superres \cite{ipol.2023.460}      & 7.05  & 0.76 & 0.46 & 8.76   & 3.66 \\
% RAFT \cite{teed2020raftrecurrentallpairsfield}          & 6.38  & 0.68 & 0.55 & 47.78  & 56.47 \\
% PWC-Net \cite{}       & - & - & - & -  & - \\
% SPyNet \cite{}          & -  & - & - & -  & - \\
% LoFTR \cite{sun2021loftrdetectorfreelocalfeature}         & 2.82  & 0.98 & 0.09 & 2.83   & 2.27 \\
% \rowcolor{green!20} Our Model    & 1.57  & 0.99 & 0.06 & 1.34   & 0.89 \\
% \midrule
% \multicolumn{6}{c}{\emph{High Exposure - 48 raw frames}} \\
% \midrule
% \cite{10.5555/1623264.1623280}   & 66.66 & 0.02 & 0.70 & 50.25  & 11.20 \\
% HDRPLUS \cite{10.1145/2980179.2980254}       & 43.70 & 0.06 & 0.70 & 34.76  & 11.40 \\
% Superres \cite{ipol.2023.460}       & 43.74 & 0.06 & 0.70 & 34.79  & 11.39 \\
% RAFT \cite{teed2020raftrecurrentallpairsfield}          & 3.88  & 0.63 & 0.61 & 49.11  & 56.97 \\
% PWC-Net \cite{}       & - & - & - & -  & - \\
% SPyNet \cite{}          & -  & - & - & -  & - \\
% LoFTR \cite{sun2021loftrdetectorfreelocalfeature}         & 2.86  & 0.96 & 0.16 & 3.04   & 2.59 \\
% \rowcolor{green!20} Our Model    & 1.76  & 0.99 & 0.05 & 1.32   & 0.75 \\
% \midrule
% \multicolumn{6}{c}{\emph{Auto Exposure - 48 raw frames}} \\
% \midrule
% \cite{10.5555/1623264.1623280}   & - & - & - & -  & - \\
% HDRPLUS \cite{10.1145/2980179.2980254}       & - & - & - & - & - \\
% Superres \cite{ipol.2023.460}       & - & - & - & -  & - \\
% RAFT \cite{teed2020raftrecurrentallpairsfield}          & -  & - & - & -  & - \\
% PWC-Net \cite{}       & - & - & - & -  & - \\
% SPyNet \cite{}          & -  & - & - & -  & - \\
% LoFTR \cite{sun2021loftrdetectorfreelocalfeature}         & -  & - & - & -   & -\\
% \rowcolor{green!20} Our Model    & -  & - & - & - & - \\
% \bottomrule
% \end{tabular}
% \end{table}
\begin{table*}[!htbp]
% \scriptsize
\centering
\renewcommand{\arraystretch}{0.8} 
\setlength{\tabcolsep}{5.0pt}
\setlength{\extrarowheight}{4pt}
\caption{Comparison of alignment methods across different exposure conditions. Each metric is shown as mean $\pm$ standard deviation where applicable.}
\label{tab:bmatch_2}
\begin{tabular}{l|ccc|ccc}
\toprule
& \multicolumn{3}{c|}{Low exposure} &\multicolumn{3}{c}{High exposure} \\
\cmidrule{2-7}
Method & \makecell{Mean$\downarrow$} & \makecell{Cosine$\uparrow$} & \makecell{Median$\downarrow$} & \makecell{Mean$\downarrow$} & \makecell{Cosine$\uparrow$} & \makecell{Median$\downarrow$} \\
\midrule
Lucas-Kanade~\cite{10.5555/1623264.1623280} & 109.35$\pm$28.02 & 0.02$\pm$0.71 & 135.91$\pm$41.43 & 50.25$\pm$11.20 & 0.02$\pm$0.70 & 69.22$\pm$15.20 \\
SPyNet~\cite{ranjan2016opticalflowestimationusing} & 75.82$\pm$27.48 & 0.05$\pm$0.70 & 110.72$\pm$45.02 & 59.64$\pm$26.94 & 0.15$\pm$0.69 & 92.74$\pm$45.66 \\
RAFT~\cite{teed2020raftrecurrentallpairsfield} & 63.70$\pm$61.19 & 0.54$\pm$0.68 & 75.85$\pm$103.93 & 49.11$\pm$56.97 & 0.63$\pm$0.61 & 54.69$\pm$97.80 \\
HDRPLUS~\cite{10.1145/2980179.2980254} & 44.92$\pm$13.10 & 0.10$\pm$0.70 & 59.63$\pm$21.73 & 34.76$\pm$11.40 & 0.06$\pm$0.70 & 47.09$\pm$13.63 \\
Deep-Burst-SR~\cite{ipol.2023.460} & 45.00$\pm$13.09 & 0.11$\pm$0.70 & 59.78$\pm$21.68 & 34.79$\pm$11.39 & 0.06$\pm$0.70 & 47.15$\pm$13.61 \\
LoFTR~\cite{sun2021loftrdetectorfreelocalfeature} & 3.94$\pm$3.04 & 0.94$\pm$0.19 & 5.95$\pm$4.76 & 3.04$\pm$2.59 & 0.96$\pm$0.16 & 4.62$\pm$4.01 \\
PWC-Net~\cite{sun2018pwcnetcnnsopticalflow} & 2.17$\pm$3.47 & 0.97$\pm$0.18 & \textbf{1.25}$\pm$\textbf{1.20} & 1.50$\pm$2.05 & 0.98$\pm$0.15 & \textbf{0.92}$\pm$\textbf{0.47} \\
 \textbf{Ours} & \textbf{1.40}$\pm$\textbf{1.15} & \textbf{0.99}$\pm$\textbf{0.06} & 2.02 $\pm$ 1.54 & \textbf{1.32}$\pm$\textbf{0.75} & \textbf{0.99}$\pm$\textbf{0.05} & 1.89 $\pm$ 0.99 \\
\bottomrule
\end{tabular}
\end{table*}




% \begin{table*}[!htbp]
% \scriptsize
% \centering
% \renewcommand{\arraystretch}{0.95} 
% \setlength{\tabcolsep}{5.0pt}
% \setlength{\extrarowheight}{4pt}
% \caption{Comparison of alignment methods across different exposure conditions. Each metric is shown as mean $\pm$ standard deviation where applicable.}
% \begin{tabular}{l|ccc|ccc|ccc}
% \toprule
% & \multicolumn{3}{c|}{Low Exposure} & \multicolumn{3}{c|}{Medium Exposure} & \multicolumn{3}{c}{High Exposure} \\
% \cmidrule{2-10}
% Method & \makecell{Mean$\downarrow$} & \makecell{Cosine$\uparrow$} & \makecell{Median$\downarrow$} & \makecell{Mean$\downarrow$} & \makecell{Cosine$\uparrow$} & \makecell{Median$\downarrow$} & \makecell{Mean$\downarrow$} & \makecell{Cosine$\uparrow$} & \makecell{Median$\downarrow$} \\
% \midrule
% Lucas-Kanade~\cite{10.5555/1623264.1623280} & 109.35$\pm$28.02 & 0.02$\pm$0.71 & 135.91$\pm$41.43 & 15.86$\pm$5.40 & 0.41$\pm$0.64 & 22.89$\pm$8.27 & 50.25$\pm$11.20 & 0.02$\pm$0.70 & 69.22$\pm$15.20 \\
% SPyNet~\cite{ranjan2016opticalflowestimationusing} & 75.82$\pm$27.48 & 0.05$\pm$0.70 & 110.72$\pm$45.02 & 2.38$\pm$1.80 & 0.97$\pm$0.16 & 2.00$\pm$1.70 & 59.64$\pm$26.94 & 0.15$\pm$0.69 & 92.74$\pm$45.66 \\
% RAFT~\cite{teed2020raftrecurrentallpairsfield} & 63.70$\pm$61.19 & 0.54$\pm$0.68 & 75.85$\pm$103.93 & 47.78$\pm$56.47 & 0.68$\pm$0.55 & 54.25$\pm$93.67 & 49.11$\pm$56.97 & 0.63$\pm$0.61 & 54.69$\pm$97.80 \\
% HDRPLUS~\cite{10.1145/2980179.2980254} & 44.92$\pm$13.10 & 0.10$\pm$0.70 & 59.63$\pm$21.73 & 8.77$\pm$3.66 & 0.76$\pm$0.45 & 9.11$\pm$6.90 & 34.76$\pm$11.40 & 0.06$\pm$0.70 & 47.09$\pm$13.63 \\
% Deep-Burst-SR~\cite{ipol.2023.460} & 45.00$\pm$13.09 & 0.11$\pm$0.70 & 59.78$\pm$21.68 & 8.76$\pm$3.66 & 0.76$\pm$0.46 & 9.10$\pm$6.90 & 34.79$\pm$11.39 & 0.06$\pm$0.70 & 47.15$\pm$13.61 \\
% LoFTR~\cite{sun2021loftrdetectorfreelocalfeature} & 3.94$\pm$3.04 & 0.94$\pm$0.19 & 5.95$\pm$4.76 & 2.83$\pm$2.27 & 0.98$\pm$0.09 & 4.29$\pm$3.47 & 3.04$\pm$2.59 & 0.96$\pm$0.16 & 4.62$\pm$4.01 \\
% PWC-Net~\cite{sun2018pwcnetcnnsopticalflow} & 2.17$\pm$3.47 & 0.97$\pm$0.18 & 1.25$\pm$1.20 & 1.66$\pm$2.64 & 0.98$\pm$0.13 & 0.93$\pm$0.49 & 1.50$\pm$2.05 & 0.98$\pm$0.15 & 0.92$\pm$0.47 \\
% \rowcolor{green!20} \textbf{Ours} & \textbf{1.40}$\pm$\textbf{1.15} & \textbf{0.99}$\pm$\textbf{0.06} & \textbf{2.02}$\pm$\textbf{1.54} & \textbf{1.34}$\pm$\textbf{0.89} & \textbf{0.99}$\pm$\textbf{0.06} & \textbf{1.92}$\pm$\textbf{1.19} & \textbf{1.32}$\pm$\textbf{0.75} & \textbf{0.99}$\pm$\textbf{0.05} & \textbf{1.89}$\pm$\textbf{0.99} \\
% \bottomrule
% \end{tabular}
% \end{table*}

==> tables/table_comparison.tex <==
% \begin{table*}[ht]
% \centering
% \caption{Comparison of different deblurring methods.}
% \begin{tabular}{lccccccc}
% \toprule
% Methods & MetaRestore-Syn & & MetaRestore-Real & & Params. (M) & MACs (G) & Time (Sec) \\
% \cmidrule(lr){2-2} \cmidrule(lr){4-5}
% & PSNR $\uparrow$ / SSIM $\uparrow$ / LPIPS $\downarrow$ / NIQE $\downarrow$  & & PSNR $\uparrow$ / SSIM $\uparrow$ / LPIPS $\downarrow$ / NIQE $\downarrow$ & & & & \\
% \midrule
% ADNet \cite{TIAN2020117} $^{*}$ & 20.48 / - & & - / - / - & & 2.81 & 203 & 0.01 \\
% HDRUNet \cite{chen2021hdrunetsingleimagehdr} $^{*}$ & - / - & & - / - / - & & - & - & - \\
% % HDR+$^{*}$  & - / - & & - / - / - & & - & - & - \\
% ESRGAN \cite{wang2018esrganenhancedsuperresolutiongenerative} $^{\dagger}$  & - / - & & - / - / - & & - & - & - \\
% DBSR \cite{bhat2021deepburstsuperresolution} $^{\dagger}$ & - / - & & - / - / - & & - & - & - \\
% HCDeblur \cite{rim2024deephybridcameradeblurring} $^{\ddagger}$ & - / - & & - / - / - & &  & - & - \\
% EIDL-DRMI \cite{seo2024deeplearningdrivenendtoendmetalensimaging} $^{\ddagger}$ & - / - & & - / - / - & & - & - & - \\
% NAFNet \cite{chen2022simplebaselinesimagerestoration} $^{\ddagger}$ & - / - & & - / - / - & & - & - & - \\
% Multi-Wiener Net $^{\ddagger}$& - / - & & - / - / - & & - & - & - \\
% DiffIR $^{\ddagger\ddagger}$& - / - & & - / - / - & & - & - & - \\
% DPIR (P$^3$) \cite{zhang2021plugandplayimagerestorationdeep} $^{\ddagger\ddagger}$& - / - & & - / - / - & & - & - & - \\
% USRNet \cite{9157092} $^{\ddagger\ddagger}$  & - / - & & - / - / - & & - & - & - \\
% % MotionETR \cite{Zhang2021} & 25.24 / 0.6951 & & 4.52 / 26.00 / 0.63 & & 10.68 & 11439 & 4.68 \\
% \textbf{Ours} & - / - & & - / - / - & & - & - & - \\
% % Ours\(_{medium}\) & - / - & & - / - / - & & - & - & - \\
% % Ours\(_{big}\) & 29.1 / - & & - / - / - & & - & - & - \\
% % Ours (big) & 26.13 / 0.7251 & & 4.11 / 25.51 / 0.67 & & 14.89 & 5189 & 2.35 \\
% % Ours & 26.76 / 0.7373 & & 3.95 / 24.65 / 0.69 & & 16.95 & 6288 & 3.85 \\
% \bottomrule
% \end{tabular}
% \end{table*}

% \begin{table*}[t]
% \centering
% \caption{Quantitative comparison of different deblurring methods on synthetic and real metalens images. Best results are shown in \textbf{bold}.}
% \renewcommand{\arraystretch}{1.2}
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{l|ccc|ccc|cc}
% \toprule
% \multirow{2}{*}{Methods} & \multicolumn{3}{c|}{MetaRestore-Syn} & \multicolumn{3}{c|}{MetaRestore-Real} & \multirow{2}{*}{\makecell{Params\\(M)}} & \multirow{2}{*}{\makecell{Time\\(s)}} \\
% \cmidrule{2-7}
% & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & & \\
% \midrule
% ADNet~\cite{TIAN2020117}$^{*}$ & 20.48 & -- & -- & -- & -- & -- & 2.81 & 0.01 \\
% HDRUNet~\cite{chen2021hdrunetsingleimagehdr}$^{*}$ & -- & -- & -- & -- & -- & -- & -- & -- \\
% ESRGAN~\cite{wang2018esrganenhancedsuperresolutiongenerative}$^{\dagger}$ & -- & -- & -- & -- & -- & -- & -- & -- \\
% DBSR~\cite{bhat2021deepburstsuperresolution}$^{\dagger}$ & -- & -- & -- & -- & -- & -- & -- & -- \\
% \midrule
% HCDeblur~\cite{rim2024deephybridcameradeblurring}$^{\ddagger}$ & -- & -- & -- & -- & -- & -- & -- & -- \\
% EIDL-DRMI~\cite{seo2024deeplearningdrivenendtoendmetalensimaging}$^{\ddagger}$ & -- & -- & -- & -- & -- & -- & -- & -- \\
% NAFNet~\cite{chen2022simplebaselinesimagerestoration}$^{\ddagger}$ & -- & -- & -- & -- & -- & -- & -- & -- \\
% Multi-Wiener Net$^{\ddagger}$ & -- & -- & -- & -- & -- & -- & -- & -- \\
% \midrule
% DiffIR$^{\ddagger\ddagger}$ & -- & -- & -- & -- & -- & -- & -- & -- \\
% DPIR~\cite{zhang2021plugandplayimagerestorationdeep}$^{\ddagger\ddagger}$ & -- & -- & -- & -- & -- & -- & -- & -- \\
% USRNet~\cite{9157092}$^{\ddagger\ddagger}$ & -- & -- & -- & -- & -- & -- & -- & -- \\
% \midrule
% \textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- \\
% \bottomrule
% \multicolumn{9}{l}{\small $^{*}$Traditional image restoration. $^{\dagger}$Learning-based restoration. $^{\ddagger}$Metalens-specific. $^{\ddagger\ddagger}$Plug-and-play methods.}
% \end{tabular}
% \vspace{-3mm}
% \label{tab:comparison}
% \end{table*}

% \begin{table*}[t]
% \centering
% \caption{Quantitative comparison of different deblurring methods on synthetic and real metalens images. Best results are shown in \textbf{bold}.}
% \renewcommand{\arraystretch}{1.0}  % Reduced from 1.2
% \setlength{\tabcolsep}{3.5pt}      % Slightly reduced horizontal spacing
% \begin{tabular}{l|cccc|cccc|ccc}
% \toprule
% \multirow{2}{*}{Methods} & \multicolumn{4}{c|}{MetaRestore-Syn} & \multicolumn{4}{c|}{MetaRestore-Real} & \multirow{2}{*}{\makecell{Params\\(M)}} & \multirow{2}{*}{\makecell{MACs\\(G)}} & \multirow{2}{*}{\makecell{Time\\(s)}} \\
% \cmidrule{2-9}
% & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & NIQE$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & NIQE$\downarrow$ & & & \\
% \midrule
% ADNet~\cite{TIAN2020117}$^{*}$ & 20.48 & -- & -- & -- & -- & -- & -- & -- & 2.81 & 203 & 0.01 \\
% HDRUNet~\cite{chen2021hdrunetsingleimagehdr}$^{*}$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% ESRGAN~\cite{wang2018esrganenhancedsuperresolutiongenerative}$^{\dagger}$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% DBSR~\cite{bhat2021deepburstsuperresolution}$^{\dagger}$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% \midrule
% HCDeblur~\cite{rim2024deephybridcameradeblurring}$^{\ddagger}$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% EIDL-DRMI~\cite{seo2024deeplearningdrivenendtoendmetalensimaging}$^{\ddagger}$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% NAFNet~\cite{chen2022simplebaselinesimagerestoration}$^{\ddagger}$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% Multi-Wiener Net$^{\ddagger}$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% \midrule
% DiffIR$^{\ddagger\ddagger}$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% DPIR~\cite{zhang2021plugandplayimagerestorationdeep}$^{\ddagger\ddagger}$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% USRNet~\cite{9157092}$^{\ddagger\ddagger}$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% \midrule
% \textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% \bottomrule
% \multicolumn{11}{l}{\small $^{*}$Traditional image restoration. $^{\dagger}$Learning-based restoration. $^{\ddagger}$Metalens-specific. $^{\ddagger\ddagger}$Plug-and-play methods.}
% \end{tabular}
% \vspace{-3mm}
% \label{tab:comparison}
% \end{table*}


% \begin{table*}[!ht]
% \small
% \centering
% \setlength{\tabcolsep}{3pt}
% \renewcommand{\arraystretch}{0.95}
% \caption{Quantitative comparison across different restoration method categories. Best results in \textbf{bold}.}
% \begin{tabular}{l|cccc|cccc|ccc}
% \toprule
% \multirow{2}{*}{Methods} & \multicolumn{4}{c|}{MetaRestore-Syn} & \multicolumn{4}{c|}{MetaRestore-Real} & \multirow{2}{*}{\makecell{Params\\(M)}} & \multirow{2}{*}{\makecell{MACs\\(G)}} & \multirow{2}{*}{\makecell{Time\\(s)}} \\
% \cmidrule{2-9}
% & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & NIQE$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & NIQE$\downarrow$ & & & \\
% \midrule
% \multicolumn{12}{l}{\textit{HDR Methods:}} \\
% ADNet~\cite{TIAN2020117} & 20.48 & -- & -- & -- & -- & -- & -- & -- & 2.81 & 203 & 0.01 \\
% HDRUNet~\cite{chen2021hdrunetsingleimagehdr} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% \midrule
% \multicolumn{12}{l}{\textit{Plug-and-Play Methods:}} \\
% DPIR~\cite{zhang2021plugandplayimagerestorationdeep} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% GSPnP & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% DiffPIR & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% \midrule
% \multicolumn{12}{l}{\textit{Super-Resolution Methods:}} \\
% Real-ESRGAN & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% USRNet~\cite{9157092} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% DBSR~\cite{bhat2021deepburstsuperresolution} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% \midrule
% \multicolumn{12}{l}{\textit{Burst Attention Fusion Methods:}} \\
% BSRT & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% EBSR & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% HCDeblur~\cite{rim2024deephybridcameradeblurring} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% \midrule
% \multicolumn{12}{l}{\textit{General Restoration Methods:}} \\
% SwinIR & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% NAFNet~\cite{chen2022simplebaselinesimagerestoration} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% Restormer & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% \midrule
% \multicolumn{12}{l}{\textit{Tailored Restoration Methods:}} \\
% Multi-Wiener Net & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% EIDL-DRMI~\cite{seo2024deeplearningdrivenendtoendmetalensimaging} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% \midrule
% \textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% \bottomrule
% \end{tabular}
% \vspace{-2mm}
% \label{tab:comparison}
% \end{table*}

% \begin{table*}[!ht]
% \small
% \centering
% \setlength{\tabcolsep}{3pt}
% \renewcommand{\arraystretch}{0.95}
% \caption{Quantitative comparison across different restoration method categories. Best results in \textbf{bold}.}
% \begin{tabular}{l|c|cccc|cccc|ccc}
% \toprule
% \multirow{2}{*}{Category} & \multirow{2}{*}{Methods} & \multicolumn{4}{c|}{\dataName{} ($\pm$ 1 EV stop)} & \multicolumn{4}{c|}{\dataName{} ($\pm$ 2 EV stop)} & \multirow{2}{*}{\makecell{Params\\(M)}} & \multirow{2}{*}{\makecell{MACs\\(G)}} & \multirow{2}{*}{\makecell{Time\\(s)}} \\
% \cmidrule{3-10}
% & & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & NIQE$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & NIQE$\downarrow$ & & & \\
% \midrule
% \multirow{6}{*}{HDR} & ADNet~\cite{TIAN2020117} & 22.34 & 0.72 & 0.35 & 5.14 & -- & -- & -- & -- & 2.81 & 203 & 0.01 \\
% & HDRUNet~\cite{chen2021hdrunetsingleimagehdr} & 18.37 & 0.62 & 0.46 & 6.09 & -- & -- & -- & -- & -- & -- & -- \\
% & AHDRNet~\cite{yan2019attention} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% & SCTNet~\cite{tel2023alignment} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% & HDR-Tran~\cite{} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% & BracketIRE~\cite{zhang2024exposure} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

% % \midrule
% % \multirow{2}{*}{\makecell[l]{Plug-and-\\Play}} & DPIR~\cite{zhang2021plugandplayimagerestorationdeep} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% % & GSPnP & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% % & DiffPIR & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% % \midrule
% \midrule
% \multirow{5}{*}{\makecell[l]{Burst\\Fusion}} & BSRT \cite{luo2022bsrt} & 24.62 & 0.76 & 0.29 & 4.91 & 23.41 & 0.73 & 0.38 & 5.74 & 19.62 & 3433 & 0.77 \\
% & EBSR \cite{luo2021ebsr} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% & DBSR~\cite{bhat2021deepburstsuperresolution} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% & USRNet~\cite{9157092} & 25.01 & 0.76 & 0.34 & 5.90 & -- & -- & -- & -- & -- & -- & -- \\
% & HCDeblur~\cite{rim2024deephybridcameradeblurring} & 21.96 & 0.71 & 0.36 & 4.63 & -- & -- & -- & -- & 9.61 & 39.11 & 0.07 \\
% \midrule
% \multirow{4}{*}{\makecell[l]{General\\Restoration}} & SwinIR \cite{liang2021swinir} & 23.24 & 0.73 & 0.31 & 4.43 & 22.10 & 0.70 & 0.43 & 5.17 & 11.47 & 1693 & 1.06 \\
% & NAFNet~\cite{chen2022simplebaselinesimagerestoration} & 21.15 & 0.68 & 0.35 & 4.93 & -- & -- & -- & -- & 29.10 & 36.39 & 0.05 \\
% & Restormer \cite{zamir2022restormer} & 26.70 & 0.81 & 0.24 & 5.04 & 26.35 & 0.79 & 0.29 & 5.80 & 26.1 & 317.6 & 0.11 \\
% & Real-ESRGAN \cite{wang2021real} & 8.57 & 0.05 & 0.68 & 12.14 & -- & -- & -- & -- & -- & -- & -- \\
% \midrule
% \multirow{3}{*}{\makecell[l]{Metalens\\Restoration}} & MultiWiener-Net \cite{yanny2022deep} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% & NeuralNano~\cite{tseng2021neural} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% & EIDL-DRMI~\cite{seo2024deeplearningdrivenendtoendmetalensimaging} & 22.10 & 0.71 & 0.33 & 5.05 & -- & -- & -- & -- & -- & -- & -- \\

% \midrule
% \multicolumn{2}{l|}{\textbf{Ours}} & 26.82 & 0.81 & 0.22 & 4.65 & -- & -- & -- & -- & 37.9 & 157.0 & 0.13 \\
% \bottomrule
% \end{tabular}
% \vspace{-2mm}
% \label{tab:comparison}
% \end{table*}

\begin{table*}[t]
\scriptsize
\centering
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{0.85}
\caption{Quantitative comparison across different restoration method categories. Best results in \textbf{bold}.}
\label{tab:comparison}
\begin{tabular}{l|c|c|cccc|cccc|ccc}
\toprule
\multirow{2}{*}{Category} & \multirow{2}{*}{Methods} & \multirow{2}{*}{Year} & \multicolumn{4}{c|}{\dataName{} ($\pm$ 1 EV stop)} & \multicolumn{4}{c|}{\dataName{} ($\pm$ 2 EV stop)} & \multirow{2}{*}{\makecell{Params\\(M)}} & \multirow{2}{*}{\makecell{MACs\\(G)}} & \multirow{2}{*}{\makecell{Time\\(s)}} \\
\cmidrule{4-11}
& & & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & NIQE$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & NIQE$\downarrow$ & & & \\
\midrule
\multirow{6}{*}{HDR} & ADNet~\cite{TIAN2020117} & 2020 & 25.97 & 0.79 & 0.28 & 5.20 & 23.24 & 0.73 & 0.36 & 5.60 & 2.81 & 812.3 & 0.01 \\
% & HDRUNet~\cite{chen2021hdrunetsingleimagehdr} & 2021 & 18.37 & 0.62 & 0.46 & 6.09 & -- & -- & -- & -- & -- & -- & -- \\
\multirow{4}{*}{HDR fusion} & AHDRNet~\cite{yan2019attention} & 2019 & 24.28 & 0.76 & 0.28 & 4.84 & 22.37 & 0.72 & 0.37 & 5.47 & 1.43 & 212.5 & 0.02 \\
& SCTNet~\cite{tel2023alignment} & 2023 & 25.37 & 0.77 & 0.26 & 4.90 & 24.21 & 0.74 & 0.32 & 5.45 & 0.95 & 144.7 & 0.94 \\
& HDR-Tran~\cite{liu2022ghost} & 2022 & 25.10 & 0.76 & 0.27 & 4.84 & 25.08 & 0.76 & 0.30 & 5.36 & 1.19 & 352.2 & 0.65 \\
& BracketIRE~\cite{zhang2024exposure} & 2024 & 25.51 & 0.79 & 0.25 & 4.81 & 23.46 & 0.73 & 0.33 & 5.31 & 9.51 & 1813 & 0.13 \\
% \midrule
% \multirow{2}{*}{\makecell[l]{Plug-and-\\Play}} & DPIR~\cite{zhang2021plugandplayimagerestorationdeep} & 2021 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% & GSPnP & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% & DiffPIR & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% \midrule
\midrule
\multirow{4}{*}{\makecell[l]{Non-HDR \\ Burst\\Fusion}} & BSRT \cite{luo2022bsrt} & 2022 & 24.62 & 0.76 & 0.29 & 4.91 & 23.41 & 0.73 & 0.38 & 5.74 & 19.62 & 3433 & 0.77 \\
& EBSR \cite{luo2021ebsr} & 2021 & 20.18 & 0.63 & 0.42 & 4.92 & 18.34 & 0.59 & 0.50 & 5.36 & 23.67 & 4242 & 0.29 \\
& DBSR~\cite{bhat2021deepburstsuperresolution} & 2021 & 24.05 & 0.76 & 0.28 & 4.87 & 22.44 & 0.71 & 0.37 & \underline{5.29} & 12.88 & 1386 & 0.10 \\
& HDR-USRNet ~\cite{lecouat2022high} & 2020 & 25.87 & 0.76 & 0.34 & 5.90 & 23.25 & 0.69 & 0.41 & 6.51 & 14.96 & 256.3 & 0.03 \\
& HCDeblur~\cite{rim2024deephybridcameradeblurring} & 2024 & 25.75 & 0.79 & 0.25 & 4.88 & 25.15 & 0.76 & 0.31 & 5.53 & 9.61 & 39.11 & 0.07 \\
\midrule
\multirow{4}{*}{\makecell[l]{General\\Restoration}} & SwinIR \cite{liang2021swinir} & 2021 & 23.24 & 0.73 & 0.31 & \textbf{4.43} & 22.10 & 0.70 & 0.43 & \textbf{5.17} & 11.47 & 1693 & 1.06 \\
& NAFNet~\cite{chen2022simplebaselinesimagerestoration} & 2022 & 26.63 & \textbf{0.81} & \underline{0.24} & 5.01 & \underline{26.37} & \underline{0.79} & \underline{0.28} &  5.64 & 29.10 & 36.39 & 0.05 \\
& Restormer \cite{zamir2022restormer} & 2022 & \underline{26.70} & \textbf{0.81} & \underline{0.24} & 5.04 & 26.35 & \underline{0.79} & 0.29 & 5.80 & 26.1 & 317.6 & 0.11 \\
& Real-ESRGAN \cite{wang2021real} & 2021 & 23.95 & 0.76 & 0.26 & 4.69 & 22.34 & 0.72 & 0.35 & 5.36 & 26.63 & 3925 & 0.3 \\
\midrule
\multirow{2}{*}{\makecell[l]{Metalens}} 

& MultiWiener-Net \cite{yanny2022deep} & 2022 & 23.41 & 0.71 & 0.35 & 4.72 & 21.31 & 0.67 & 0.42 & 5.90 & 3.32 & 49.57 & 0.01 \\
% % & NeuralNano~\cite{tseng2021neural} & 2021 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& EIDL-DRMI~\cite{seo2024deeplearningdrivenendtoendmetalensimaging} & 2024 & 23.50 & 0.74 & 0.25 & 4.78 & 21.45 & 0.68 & 0.31 & 5.59 & 29.10 & 36.39 & 0.05 \\
\midrule
\rowcolor{green!20} \multicolumn{2}{l|}{\textbf{Ours}} & 2025 & \textbf{26.82} & \textbf{0.81} & \textbf{0.22} & \underline{4.65} & \textbf{26.52} & \textbf{0.79} & \textbf{0.25} & 5.53 & 37.9 & 157.0 & 0.13 \\
\bottomrule
\end{tabular}
% \vspace{-2mm}
\end{table*}

==> tables/table_dataset.tex <==
\begin{table}[h!]
\centering
\caption{MetaHDR Dataset Composition}
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.8}
\begin{tabular}{@{}cccp{2cm}c@{}}
\toprule
\textbf{Dataset} & \textbf{Size} & \textbf{\#Burst} & \textbf{Scenes} & \textbf{Train\%} \\
\midrule
\multicolumn{5}{l}{\textit{Burst HDR Datasets}} \\
\midrule
Burst-HDR+ \cite{hasinoff2016burst} & 3750 & 2-10 & Indoor/outdoor, day/night & 80\% \\
Kalantari et al. \cite{kalantari2017deep} & 222 & 3 & Indoor/outdoor, person, motion & 90\% \\
\midrule
\multicolumn{5}{l}{\textit{Non-Burst HDR Datasets}} \\
\midrule
HDM-HDR \cite{froehlich2014creating} & 423 & N/A & Outdoor, Night, extreme bright/dark & 90\% \\
Zurich Raw \cite{ignatov2020replacing} & 504 & N/A & Outdoor driving & 85\% \\
\midrule
\multicolumn{5}{l}{\textit{Non-Burst Image Datasets}} \\
\midrule
Flickr2K & 2650 & N/A & General scenes & 70\% \\
Div2K \cite{Agustsson_2017_CVPR_Workshops} & 800 & N/A & General scenes & 70\% \\
Liu4K \cite{Liu4K} & 1600 & N/A & Ultra high-res scenes & 70\% \\
\midrule
\multicolumn{5}{l}{\textit{Real metalens images (for unsupervised finetuning)}} \\
\midrule
MetaHDR & 200 & 5-20 & Indoor/outdoor, dark/bright, direct illumination/shade & 100\% \\
\bottomrule
\end{tabular}
\label{table:data}
\end{table}
